Provably Powerful Graph Neural Networks for Directed Multigraphs

This paper analyses a set of simple adaptations that transform standard message-passing Graph Neural Networks (GNN) into provably powerful directed multigraph neural networks. The adaptations include multigraph port numbering, ego IDs, and reverse message passing. We prove that the combination of these theoretically enables the detection of any directed subgraph pattern. To validate the effectiveness of our proposed adaptations in practice, we conduct experiments on synthetic subgraph detection tasks, which demonstrate outstanding performance with almost perfect results. Moreover, we apply our proposed adaptations to two financial crime analysis tasks. We observe dramatic improvements in detecting money laundering transactions, improving the minority-class F1 score of a standard message-passing GNN by up to 30%, and closely matching or outperforming tree-based and GNN baselines. Similarly impressive results are observed on a real-world phishing detection dataset, boosting three standard GNNs' F1 scores by around 15% and outperforming all baselines.

==> Rebuttal/AML_collapse_and_random_ports.tex <==
\begin{tabular}{lrr}
\toprule
{Model} & AML Small HI & AML Small LI \\
\midrule

GIN & 
\cellcolor[HTML]{b8e3b2} \color[HTML]{000000} $39.31 \pm 4.86$ & \cellcolor[HTML]{d3eecd} \color[HTML]{000000} $33.09 \pm 3.86$ \\
{\ +ReverseMP} & 
\cellcolor[HTML]{097532} \color[HTML]{f1f1f1} $74.78 \pm 13.96$ & \cellcolor[HTML]{66bd6f} \color[HTML]{f1f1f1} $54.63 \pm 6.09$ \\
{\ +ReverseMP+Ports(random)} & 
\cellcolor[HTML]{006227} \color[HTML]{f1f1f1} $79.01 \pm 2.86$ & \cellcolor[HTML]{4aaf61} \color[HTML]{f1f1f1} $59.15 \pm 6.86$ \\
{\ +ReverseMP+Ports} & 
\cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} $84.90 \pm 2.08$ & \cellcolor[HTML]{289049} \color[HTML]{f1f1f1} $67.39 \pm 3.18$ \\
{\ +ReverseMP+Ports+EgoIDs} & 
\cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} $84.26 \pm 2.93$ & \cellcolor[HTML]{289049} \color[HTML]{f1f1f1} $67.41 \pm 2.86$ \\
$\text{GIN}^{\text{c}}$ & 
\cellcolor[HTML]{eff9ec} \color[HTML]{000000} $23.79 \pm 4.86$ & \cellcolor[HTML]{f4fbf1} \color[HTML]{000000} $21.69 \pm 5.90$ \\
$\text{GIN+ReverseMP+Ports}^{\text{c}}$ & 
\cellcolor[HTML]{dbf1d6} \color[HTML]{000000} $30.67 \pm 3.57$ & \cellcolor[HTML]{e5f5e1} \color[HTML]{000000} $27.91 \pm 7.73$ \\
\bottomrule
\end{tabular}

==> Rebuttal/SIM_condensed.tex <==
\begingroup
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
Model & C2 & C3 & C4 & C5 & C6 \\
\midrule
GIN & 
% \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.58 & 
% \cellcolor[HTML]{00682a} \color[HTML]{f1f1f1} 95.57 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 35.91 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 34.67 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 58.00 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 50.80 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.12 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.59 & 
% \cellcolor[HTML]{cbebc5} \color[HTML]{000000} 69.31 & 
% \cellcolor[HTML]{ecf8e8} \color[HTML]{000000} 63.12 
\\
GIN+randomIDs& 
% \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.68 & 
% \cellcolor[HTML]{006b2b} \color[HTML]{f1f1f1} 95.26 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 40.72 &
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.05 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.30 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 46.73 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.61 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.32 & 
% \cellcolor[HTML]{dff3da} \color[HTML]{000000} 65.97 & 
% \cellcolor[HTML]{ebf7e7} \color[HTML]{000000} 63.58 
\\
% GAT & 
% % \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 10.33 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 10.53 & 
% % \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  9.69 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.86 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 \\
% PNA & 
% % \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.63 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.02 & 
% % \cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} 95.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 38.93 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.77 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.75 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.92 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.79 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.40 & \cellcolor[HTML]{e0f3db} \color[HTML]{000000} 65.88 & 
% \cellcolor[HTML]{e2f4dd} \color[HTML]{000000} 65.51 \\
% GIN+EU \citep{battaglia2018relational_edgeupdates} &
% % , cardoso2022laundrograph} & 
% \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.30 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.74 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.70 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.13 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 32.58 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.65 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.62 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.68 & \cellcolor[HTML]{d0edca} \color[HTML]{000000} 68.54 & \cellcolor[HTML]{e7f6e2} \color[HTML]{000000} 64.64 \\
\midrule
GIN+EgoIDs & 
% \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.78 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.48 & 
% \cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} 95.06 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.24 & 
\cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.13 & \cellcolor[HTML]{005321} \color[HTML]{f1f1f1} 97.97 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 53.12 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.37 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.42 & 
% \cellcolor[HTML]{dcf2d7} \color[HTML]{000000} 66.44 & 
% \cellcolor[HTML]{e9f7e5} \color[HTML]{000000} 63.90 
\\
% GIN+EdgeUpdates & 
% \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.30 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.74 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.70 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.13 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 32.58 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.65 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.62 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.68 & \cellcolor[HTML]{d0edca} \color[HTML]{000000} 68.54 & \cellcolor[HTML]{e7f6e2} \color[HTML]{000000} 64.64 \\
GIN+Ports & 
% \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.47 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.00 & 
% \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.59 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 41.51 &
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 27.79 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 56.11 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.68 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 41.11 & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.99 & 
% \cellcolor[HTML]{d3eecd} \color[HTML]{000000} 67.99 & 
% \cellcolor[HTML]{e1f3dc} \color[HTML]{000000} 65.76 
\\
% \midrule
% GIN+ReverseMP & 
% % \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.87 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.08 & 
% % \cellcolor[HTML]{006d2c} \color[HTML]{f1f1f1} 94.99 & \cellcolor[HTML]{006b2b} \color[HTML]{f1f1f1} 95.25 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 35.96 & \cellcolor[HTML]{e9f7e5} \color[HTML]{000000} 63.85 & 
% \cellcolor[HTML]{ccebc6} \color[HTML]{000000} 69.09 & \cellcolor[HTML]{d7efd1} \color[HTML]{000000} 67.44 & 
% \cellcolor[HTML]{bee5b8} \color[HTML]{000000} 71.23 & 
% % \cellcolor[HTML]{e0f3db} \color[HTML]{000000} 65.83 & 
% % \cellcolor[HTML]{def2d9} \color[HTML]{000000} 66.18 
% \\
% {\ +Ports} & 
% % \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.41 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.35 & 
% % \cellcolor[HTML]{005020} \color[HTML]{f1f1f1} 98.51 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.16 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.15 & \cellcolor[HTML]{ebf7e7} \color[HTML]{000000} 63.58 & 
% \cellcolor[HTML]{cdecc7} \color[HTML]{000000} 69.00 & \cellcolor[HTML]{c4e8bd} \color[HTML]{000000} 70.35 & 
% \cellcolor[HTML]{a0d99b} \color[HTML]{000000} 75.04 & 
% % \cellcolor[HTML]{d4eece} \color[HTML]{000000} 67.84 & 
% % \cellcolor[HTML]{e1f3dc} \color[HTML]{000000} 65.78 
% \\
{GIN+EgoIDs+Ports} & 
% \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.48 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.09 & 
% \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.62 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.32 & 
\cellcolor[HTML]{004c1e} \color[HTML]{f1f1f1} 98.97 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & 
\cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.46 & \cellcolor[HTML]{17813d} \color[HTML]{f1f1f1} 91.60 & 
\cellcolor[HTML]{48ae60} \color[HTML]{f1f1f1} 84.23 & 
% \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.42 & 
% \cellcolor[HTML]{05712f} \color[HTML]{f1f1f1} 94.33 
\\
{\ \ +MoreData} & 
\cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 100.00 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 100.00 & 
\cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.96 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.80 & 
\cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 99.36 & 
% - & 
% -  
\\
% +EdgeUpdates & 
% \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.55 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.76 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.37 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.73 & \cellcolor[HTML]{2d954d} \color[HTML]{f1f1f1} 88.38 & \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.81 & \cellcolor[HTML]{005522} \color[HTML]{f1f1f1} 97.82 \\
% \midrule
% GAT+Adaptations & 
% \cellcolor[HTML]{005020} \color[HTML]{f1f1f1} 98.44 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.66 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.18 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.11 & \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.28 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.42 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.35 & \cellcolor[HTML]{026f2e} \color[HTML]{f1f1f1} 94.55 & \cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} 91.75 & \cellcolor[HTML]{218944} \color[HTML]{f1f1f1} 90.21 & \cellcolor[HTML]{79c67a} \color[HTML]{000000} 79.52 \\
% Multi-GAT & 
% % \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.68 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.36 & 
% % \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.28 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.33 & 
% \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.61 & \cellcolor[HTML]{004c1e} \color[HTML]{f1f1f1} 98.93 & 
% \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.90 & \cellcolor[HTML]{006529} \color[HTML]{f1f1f1} 95.82 & 
% \cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} 91.81 & \cellcolor[HTML]{005f26} \color[HTML]{f1f1f1} 96.66 & 
% \cellcolor[HTML]{359e53} \color[HTML]{f1f1f1} 86.92 \\
% Multi-PNA & 
% % \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.64 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.25 & 
% % \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.41 & 
% \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.54 & 
% \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.49 & \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.46 & 
% \cellcolor[HTML]{2a924a} \color[HTML]{f1f1f1} 88.75 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.07 & 
% \cellcolor[HTML]{005e26} \color[HTML]{f1f1f1} 96.77 \\
% Multi-GIN+EU & 
% \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.55 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.76 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.37 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.73 & \cellcolor[HTML]{2d954d} \color[HTML]{f1f1f1} 88.38 & \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.81 & \cellcolor[HTML]{005522} \color[HTML]{f1f1f1} 97.82 \\
% \midrule
% GIN+randomIDs& 
% % \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.68 & 
% % \cellcolor[HTML]{006b2b} \color[HTML]{f1f1f1} 95.26 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 40.72 &
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.05 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.30 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 46.73 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.61 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.32 & 
% % \cellcolor[HTML]{dff3da} \color[HTML]{000000} 65.97 & 
% % \cellcolor[HTML]{ebf7e7} \color[HTML]{000000} 63.58 
% \\
% GIN+EgoIDs & 
% % \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.82 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 52.56 & 
% % \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.67 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.78 & 
% \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.67 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.78 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.56 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.95 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.01 & \cellcolor[HTML]{cdecc7} \color[HTML]{000000} 69.00 & 
% \cellcolor[HTML]{e5f5e1} \color[HTML]{000000} 64.93 \\
% {\ +ReverseMP} & 
% % \cellcolor[HTML]{005020} \color[HTML]{f1f1f1} 98.58 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.24 & 
% % \cellcolor[HTML]{0c7735} \color[HTML]{f1f1f1} 93.19 & \cellcolor[HTML]{05712f} \color[HTML]{f1f1f1} 94.23 & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 38.18 & \cellcolor[HTML]{eef8ea} \color[HTML]{000000} 62.62 & 
% \cellcolor[HTML]{c9eac2} \color[HTML]{000000} 69.74 & \cellcolor[HTML]{ccebc6} \color[HTML]{000000} 69.08 & 
% \cellcolor[HTML]{a8dca2} \color[HTML]{000000} 74.07 & 
% % \cellcolor[HTML]{e0f3db} \color[HTML]{000000} 65.83 & 
% % \cellcolor[HTML]{eaf7e6} \color[HTML]{000000} 63.67 
% \\
\bottomrule
\end{tabular}
}
\endgroup


==> Rebuttal/new_models.tex <==
\begin{tabular}{lccccc}
\toprule
{Model} & AML Small HI   & AML Small LI   & AML Medium HI   & AML Medium LI   & ETH \\
\midrule
R-GCN   & $37.72$        & $21.20$        & $44.77$         & $21.24$         & $0.0$  \\

Di-GCN  & $15.87$        & $9.17$         & $21.78$         & $10.07$         & $0.0$ \\

MagNet  & $19.03$        & $20.99$        & $38.25$         & $22.20$         & $33.54$ \\
\midrule
Multi-GNN (best)  & $\bm{84.90}$        & $\bm{67.41}$        & $\bm{82.92}$         & $\bm{47.07}$         & $\bm{65.28}$ \\
\bottomrule
\end{tabular}

==> Rebuttal/old_datasets.tex <==
\begin{tabular}{lcccc}
\toprule
{Model}         &               Squirrel &             Chameleon &            Arxiv-Year &          Roman-Empire \\
\midrule
% FSGNN           &       $74.10 \pm 1.89$ &      $78.27 \pm 1.28$ &      $50.47 \pm 0.21$ &      $79.92 \pm 0.56$ \\
Grad. Gating    &       $64.26 \pm 2.38$ &      $71.40 \pm 2.38$ &      $63.30 \pm 1.84$ &      $82.16 \pm 0.78$ \\
\midrule
Di-GCN          &       $37.74 \pm 1.54$ &      $52.24 \pm 3.65$ &                     - &      $52.71 \pm 0.32$ \\
MagNet          &       $39.01 \pm 1.93$ &      $58.22 \pm 2.87$ &      $60.29 \pm 0.27$ &      $88.07 \pm 0.27$ \\
% Dir-GNN         &   $\bm{75.31 \pm 1.92}$&      $79.71 \pm 1.26$ &      $64.08 \pm 0.26$ &      $91.23 \pm 0.32$ \\
\midrule
GIN             &       $55.62 \pm 2.01$ &      $72.26 \pm 1.08$ &      $54.70 \pm 0.67$ &      $92.11 \pm 0.34$ \\
{\ +ReverseMP}  &       $67.72 \pm 2.08$ &      $81.80 \pm 1.23$ &      $67.77 \pm 0.30$ &      $94.86 \pm 0.24$ \\
{\ +Ports}      &       $72.59 \pm 2.40$ &      $84.47 \pm 0.82$ &  $\bm{73.22 \pm 0.51}$&  $\bm{95.75 \pm 0.20}$\\
{\ +EgoIDs}     &       $72.66 \pm 2.49$ &  $\bm{85.53 \pm 2.83}$&      $71.54 \pm 0.60$ &      $95.55 \pm 0.32$ \\
\bottomrule
\end{tabular}


==> Rebuttal2/AML_pattern_types.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
Dataset & Model 
& Fan-in 
& Fan-out 
& Cycle 
% & Gather-Scatter 
& S-G 
& B-C 
% & Stack 
% & Random 
\\
\midrule
Small HI & Multi-PNA 
& \cellcolor[HTML]{067230} \color[HTML]{f1f1f1} 85.37 
& \cellcolor[HTML]{005a24} \color[HTML]{f1f1f1} 93.13 
& \cellcolor[HTML]{45ad5f} \color[HTML]{f1f1f1} 61.62 
% & \cellcolor[HTML]{005b25} \color[HTML]{f1f1f1} 92.65 
& \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 93.72 
& \cellcolor[HTML]{62bb6d} \color[HTML]{f1f1f1} 54.55 
% & \cellcolor[HTML]{48ae60} \color[HTML]{f1f1f1} 60.68 
% & \cellcolor[HTML]{3aa357} \color[HTML]{f1f1f1} 65.48 
\\
Small HI & Multi-GIN 
& \cellcolor[HTML]{00692a} \color[HTML]{f1f1f1} 88.62 
& \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 95.42 
& \cellcolor[HTML]{55b567} \color[HTML]{f1f1f1} 57.58 
% & \cellcolor[HTML]{005622} \color[HTML]{f1f1f1} 94.49 
& \cellcolor[HTML]{00692a} \color[HTML]{f1f1f1} 88.28 
& \cellcolor[HTML]{55b567} \color[HTML]{f1f1f1} 57.58 
% & \cellcolor[HTML]{48ae60} \color[HTML]{f1f1f1} 60.68 
% & \cellcolor[HTML]{157f3b} \color[HTML]{f1f1f1} 79.76 
\\
Small LI & Multi-PNA 
& \cellcolor[HTML]{2c944c} \color[HTML]{f1f1f1} 71.43 
& \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 95.65 
& \cellcolor[HTML]{aedea7} \color[HTML]{000000} 33.33 
% & \cellcolor[HTML]{005622} \color[HTML]{f1f1f1} 94.29 
& \cellcolor[HTML]{2c944c} \color[HTML]{f1f1f1} 71.19 
& \cellcolor[HTML]{3da65a} \color[HTML]{f1f1f1} 64.29 
% & \cellcolor[HTML]{63bc6e} \color[HTML]{f1f1f1} 54.17 
% & \cellcolor[HTML]{56b567} \color[HTML]{f1f1f1} 57.14 
\\
Small LI & Multi-GIN 
& \cellcolor[HTML]{8ed08b} \color[HTML]{000000} 42.86 
& \cellcolor[HTML]{077331} \color[HTML]{f1f1f1} 84.78 
& \cellcolor[HTML]{97d492} \color[HTML]{000000} 40.48 
% & \cellcolor[HTML]{2f974e} \color[HTML]{f1f1f1} 70.00 
& \cellcolor[HTML]{6abf71} \color[HTML]{000000} 52.54 
& \cellcolor[HTML]{a7dba0} \color[HTML]{000000} 35.71 
% & \cellcolor[HTML]{bbe4b4} \color[HTML]{000000} 29.17 
% & \cellcolor[HTML]{7dc87e} \color[HTML]{000000} 47.62 
\\
\bottomrule
\end{tabular}


==> Rebuttal2/SIM_new.tex <==
\begin{tabular}{lccccccccccc}
\toprule
Model 
% & deg-in & deg-out & fan-in & fan-out & C2 & C3 
& C4 & C5 & C6 & S-G & B-C \\
\midrule
DropGIN
% & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 52.30 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.36 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.26 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.58 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 33.85 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.73 
& \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 16.92 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 26.02 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.17 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.87 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.59 \\
Multi-DropGIN
% & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 100.00 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.96 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.92 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.90 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 100.00 & \cellcolor[HTML]{00441b} \color[HTML]{f1f1f1} 99.92 
& \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.09 & \cellcolor[HTML]{005b25} \color[HTML]{f1f1f1} 97.08 & \cellcolor[HTML]{006d2c} \color[HTML]{f1f1f1} 94.93 & \cellcolor[HTML]{005c25} \color[HTML]{f1f1f1} 96.98 & \cellcolor[HTML]{05712f} \color[HTML]{f1f1f1} 94.27 \\
R-GCN
% & \cellcolor[HTML]{b2e0ac} \color[HTML]{000000} 72.76 & \cellcolor[HTML]{c0e6b9} \color[HTML]{000000} 70.96 & \cellcolor[HTML]{caeac3} \color[HTML]{000000} 69.58 & \cellcolor[HTML]{d8f0d2} \color[HTML]{000000} 67.28 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 23.20 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 58.81 
& \cellcolor[HTML]{e2f4dd} \color[HTML]{000000} 65.57 & \cellcolor[HTML]{e8f6e3} \color[HTML]{000000} 64.35 & \cellcolor[HTML]{bde5b6} \color[HTML]{000000} 71.27 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 59.23 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.61 \\
Multi-R-GCN
% & \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.15 & \cellcolor[HTML]{005321} \color[HTML]{f1f1f1} 98.01 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.11 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.08 & \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.13 & \cellcolor[HTML]{05712f} \color[HTML]{f1f1f1} 94.29 
& \cellcolor[HTML]{3fa95c} \color[HTML]{f1f1f1} 85.20 & \cellcolor[HTML]{a8dca2} \color[HTML]{000000} 74.08 & \cellcolor[HTML]{a7dba0} \color[HTML]{000000} 74.30 & \cellcolor[HTML]{5bb86a} \color[HTML]{f1f1f1} 82.37 & \cellcolor[HTML]{d9f0d3} \color[HTML]{000000} 67.16 \\
PPGN
% & \cellcolor[HTML]{dcf2d7} \color[HTML]{000000} 66.53 & \cellcolor[HTML]{dcf2d7} \color[HTML]{000000} 66.46 & \cellcolor[HTML]{e4f5df} \color[HTML]{000000} 65.18 & \cellcolor[HTML]{e8f6e3} \color[HTML]{000000} 64.36 & \cellcolor[HTML]{edf8ea} \color[HTML]{000000} 62.77 & \cellcolor[HTML]{dbf1d5} \color[HTML]{000000} 66.75 
& \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 57.93 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.74 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 41.15 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.23 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.98 \\
Multi-PPGN$^*$
% & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.68 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.66 & \cellcolor[HTML]{006428} \color[HTML]{f1f1f1} 96.00 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.72 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.51 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.56 
& \cellcolor[HTML]{005321} \color[HTML]{f1f1f1} 98.11 & \cellcolor[HTML]{127c39} \color[HTML]{f1f1f1} 92.49 & \cellcolor[HTML]{37a055} \color[HTML]{f1f1f1} 86.69 & \cellcolor[HTML]{cfecc9} \color[HTML]{000000} 68.74 & \cellcolor[HTML]{edf8ea} \color[HTML]{000000} 62.78 \\
\midrule
Multi-PNA 
% & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.64 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.25 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.41 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.54 
& \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.49 & \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.46 & \cellcolor[HTML]{2a924a} \color[HTML]{f1f1f1} 88.75 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.07 & \cellcolor[HTML]{005e26} \color[HTML]{f1f1f1} 96.77 \\
\bottomrule
\end{tabular}

==> Tables/AML_results_new.tex <==
\begin{tabular}{lcccc}
\toprule
{Model} & 
AML Small HI & 
AML Small LI & 
AML Medium HI & 
% AML Medium LI & 
ETH
%{} &  &  & (low IR) & (low IR) & 
\\
\midrule

% MLP & 
% \cellcolor[HTML]{b1e0ab} \color[HTML]{000000} $24.11 \pm 1.47$ &
% \cellcolor[HTML]{d5efcf} \color[HTML]{000000} $14.59 \pm 2.08$ &
% \cellcolor[HTML]{a0d99b} \color[HTML]{000000} $28.16 \pm 6.97$ &
% % \cellcolor[HTML]{e8f6e3} \color[HTML]{000000} $7.95 \pm 1.11$ &
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.10 \pm 0.00$ 
% \\

% MLP & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.00 \pm 0.00$ & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.00 \pm 0.00$ & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.00 \pm 0.00$ & 
% % \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.00 \pm 0.00$ & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $0.00 \pm 0.00$ 
% \\

LightGBM+GFs \citep{altman2023realistic} & 
\cellcolor[HTML]{0a7633} \color[HTML]{f1f1f1} $62.86 \pm 0.25$ & 
\cellcolor[HTML]{bee5b8} \color[HTML]{000000} $20.83 \pm 1.50$ & 
\cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} $59.48 \pm 0.15$ & 
% \cellcolor[HTML]{bee5b8} \color[HTML]{000000} $20.85 \pm 0.38$ &
\cellcolor[HTML]{2d954d} \color[HTML]{f1f1f1} $53.20 \pm 0.60$ 
\\
XGBoost+GFs \citep{altman2023realistic} & 
\cellcolor[HTML]{097532} \color[HTML]{f1f1f1} $63.23 \pm 0.17$ & 
\cellcolor[HTML]{a4da9e} \color[HTML]{000000} $27.30 \pm 0.33$ & 
\cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} $65.70 \pm 0.26$ & 
% \cellcolor[HTML]{a0d99b} \color[HTML]{000000} $28.16 \pm 0.14$ &
\cellcolor[HTML]{39a257} \color[HTML]{f1f1f1} $49.40 \pm 0.54$
\\


GIN \citep{xu2018powerful, hu2019strategies} & 
\cellcolor[HTML]{9fd899} \color[HTML]{000000} $28.70 \pm 1.13$ & 
\cellcolor[HTML]{e8f6e4} \color[HTML]{000000} $7.90 \pm 2.78$ & 
\cellcolor[HTML]{5ab769} \color[HTML]{f1f1f1} $42.20 \pm 0.44$ & 
% \cellcolor[HTML]{f2faef} \color[HTML]{000000} $2.80 \pm 3.27$ & 
\cellcolor[HTML]{a7dba0} \color[HTML]{000000} $26.92 \pm 7.52$
\\
% GAT \citep{velivckovic2017graph} & 
% \cellcolor[HTML]{c8e9c1} \color[HTML]{000000} $36.17 \pm 7.74$ & 
% \cellcolor[HTML]{ebf7e7} \color[HTML]{000000} $25.67 \pm 7.07$ & 
% \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} $15.66 \pm 20.22$ & 
% \cellcolor[HTML]{f1f1f1} \color[HTML]{000000} $4.90 \pm 7.52$ & 
% \cellcolor[HTML]{d0edca} \color[HTML]{000000} $15.94 \pm 3.89$ 
% \\
PNA \citep{velickovic2019deep} & 
\cellcolor[HTML]{218944} \color[HTML]{f1f1f1} $56.77 \pm 2.41$ & 
\cellcolor[HTML]{d4eece} \color[HTML]{000000} $14.85 \pm 1.46$ & 
\cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} $59.71 \pm 1.91$ & 
% \cellcolor[HTML]{9ed798} \color[HTML]{000000} $28.96 \pm 2.05$ & 
\cellcolor[HTML]{329b51} \color[HTML]{f1f1f1} $51.49 \pm 4.26$
\\
GIN+EU \citep{battaglia2018relational_edgeupdates} & 
\cellcolor[HTML]{3fa85b} \color[HTML]{f1f1f1} $47.73 \pm 7.86$ & 
\cellcolor[HTML]{c0e6b9} \color[HTML]{000000} $20.62 \pm 2.41$ & 
\cellcolor[HTML]{39a257} \color[HTML]{f1f1f1} $49.26 \pm 4.02$ & 
% \cellcolor[HTML]{ecf8e8} \color[HTML]{000000}  $5.95 \pm 8.32$ & 
\cellcolor[HTML]{86cc85} \color[HTML]{000000} $33.92 \pm 7.34$
\\
R-GCN \citep{schlichtkrull2018modelingRelGNN} &
\cellcolor[HTML]{5db96b} \color[HTML]{f1f1f1} $41.78 \pm 0.48$ & 
\cellcolor[HTML]{e9f7e5} \color[HTML]{000000} $7.43 \pm 0.38$ & 
OOM & 
% OOM & 
OOM 
\\


\midrule

GIN+EgoIDs \citep{you2021identity} & 
\cellcolor[HTML]{68be70} \color[HTML]{000000} $39.65 \pm 4.73$ & 
\cellcolor[HTML]{d3eecd} \color[HTML]{000000}  $14.98 \pm 2.66$ & 
\cellcolor[HTML]{4aaf61} \color[HTML]{f1f1f1} $45.26 \pm 2.16$ & 
% \cellcolor[HTML]{dff3da} \color[HTML]{000000} $11.17 \pm 0.64$ & 
\cellcolor[HTML]{aadda4} \color[HTML]{000000} $26.01 \pm 2.27$
\\
GIN+Ports \citep{sato2019approximation_port_numbers} & 
\cellcolor[HTML]{278f48} \color[HTML]{f1f1f1} $54.85 \pm 0.89$ & 
\cellcolor[HTML]{bce4b5} \color[HTML]{000000} $21.41 \pm 2.40$ & 
\cellcolor[HTML]{29914a} \color[HTML]{f1f1f1} $54.22 \pm 1.94$ & 
% \cellcolor[HTML]{e2f4dd} \color[HTML]{000000} $10.51 \pm 12.82$& 
\cellcolor[HTML]{8ace88} \color[HTML]{000000} $32.96 \pm 0.25$
\\


\midrule

GIN+ReverseMP \citep{jaume2019edgnnbidirecibmmaria} & 
\cellcolor[HTML]{42ab5d} \color[HTML]{f1f1f1} $46.79 \pm 4.97$ & 
\cellcolor[HTML]{d0edca} \color[HTML]{000000} $15.98 \pm 4.39$ & 
\cellcolor[HTML]{309950} \color[HTML]{f1f1f1} $51.93 \pm 2.90$ & 
% \cellcolor[HTML]{d7efd1} \color[HTML]{000000} $14.00 \pm 9.34$ & 
\cellcolor[HTML]{78c679} \color[HTML]{000000} $36.86 \pm 8.12$
\\
{\ +Ports} & 
\cellcolor[HTML]{208843} \color[HTML]{f1f1f1} $56.85 \pm 2.64$ & 
\cellcolor[HTML]{b2e0ac} \color[HTML]{000000} $23.80 \pm 4.07$ & 
\cellcolor[HTML]{1f8742} \color[HTML]{f1f1f1} $57.15 \pm 0.76$ & 
% \cellcolor[HTML]{dff3da} \color[HTML]{000000} $11.39 \pm 8.39$ & 
\cellcolor[HTML]{58b668} \color[HTML]{f1f1f1} $42.51 \pm 7.16$
\\
{\ +EgoIDs (Multi-GIN)} & 
\cellcolor[HTML]{1f8742} \color[HTML]{f1f1f1} $57.15 \pm 4.97$ & 
\cellcolor[HTML]{b2e0ac} \color[HTML]{000000} $23.91 \pm 1.97$ & 
\cellcolor[HTML]{238b45} \color[HTML]{f1f1f1} $56.23 \pm 1.51$ & 
% \cellcolor[HTML]{caeac3} \color[HTML]{000000} $18.10 \pm 1.35$ & 
\cellcolor[HTML]{56b567} \color[HTML]{f1f1f1} $42.86 \pm 2.53$
\\


\midrule

% Multi-GAT & 
% \cellcolor[HTML]{94d390} \color[HTML]{000000} $46.79 \pm 9.26$ & 
% \cellcolor[HTML]{e5f5e0} \color[HTML]{000000} $27.02 \pm 2.38$ & 
% \cellcolor[HTML]{e0f3db} \color[HTML]{000000} $30.27 \pm 10.57$ & 
% \cellcolor[HTML]{f1f1f1} \color[HTML]{000000} $3.15 \pm 4.04$ & 
% \cellcolor[HTML]{43ac5e} \color[HTML]{f1f1f1} $46.36 \pm 0.74$ 
% \\
Multi-PNA & 
\cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} $65.61 \pm 1.21$ & 
\cellcolor[HTML]{98d594} \color[HTML]{000000} $29.88 \pm 6.74$ & 
\cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} $65.77 \pm 1.09$ & 
% \cellcolor[HTML]{f1f1f1} \color[HTML]{000000}              nan & 
\cellcolor[HTML]{016e2d} \color[HTML]{f1f1f1} $65.28 \pm 2.89$
\\
Multi-PNA+EU & 
\cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} $65.61 \pm 1.21$ & 
\cellcolor[HTML]{98d594} \color[HTML]{000000} $29.88 \pm 6.74$ & 
\cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} $65.77 \pm 1.09$ & 
% \cellcolor[HTML]{f1f1f1} \color[HTML]{000000}              nan & 
\cellcolor[HTML]{016e2d} \color[HTML]{f1f1f1} $65.28 \pm 2.89$
\\
Multi-GIN+EU & 
\cellcolor[HTML]{1d8640} \color[HTML]{f1f1f1} $57.75 \pm 1.95$ & 
\cellcolor[HTML]{b6e2af} \color[HTML]{000000} $22.88 \pm 1.59$ & 
\cellcolor[HTML]{1e8741} \color[HTML]{f1f1f1} $57.68 \pm 6.65$ & 
% \cellcolor[HTML]{ebf7e7} \color[HTML]{000000}  $6.61 \pm 6.89$ & 
\cellcolor[HTML]{3ca559} \color[HTML]{f1f1f1} $48.37 \pm 6.62$
\\


\bottomrule
\end{tabular}




==> Tables/SIM_results.tex <==
\begingroup
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
Model & deg-in & deg-out & fan-in & fan-out & C2 & C3 & C4 & C5 & C6 & S-G & B-C \\
\midrule
GIN \citep{xu2018powerful, hu2019strategies} & 
\cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.58 & \cellcolor[HTML]{00682a} \color[HTML]{f1f1f1} 95.57 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 35.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 34.67 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 58.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 50.80 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.12 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.59 & \cellcolor[HTML]{cbebc5} \color[HTML]{000000} 69.31 & \cellcolor[HTML]{ecf8e8} \color[HTML]{000000} 63.12 \\
GAT \citep{velivckovic2017graph} & 
\cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 10.33 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 10.53 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  9.69 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.86 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000}  0.00 \\
PNA \citep{velickovic2019deep} & 
\cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.63 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 43.02 & \cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} 95.00 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 38.93 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 25.77 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.75 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.92 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.79 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 48.40 & \cellcolor[HTML]{e0f3db} \color[HTML]{000000} 65.88 & \cellcolor[HTML]{e2f4dd} \color[HTML]{000000} 65.51 \\
GIN+EU \citep{battaglia2018relational_edgeupdates} &
% , cardoso2022laundrograph} & 
\cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.30 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.74 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.70 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.13 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 32.58 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.65 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.62 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.68 & \cellcolor[HTML]{d0edca} \color[HTML]{000000} 68.54 & \cellcolor[HTML]{e7f6e2} \color[HTML]{000000} 64.64 \\
\midrule
GIN+EgoIDs \citep{you2021identity} & 
\cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.78 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 51.48 & \cellcolor[HTML]{006c2c} \color[HTML]{f1f1f1} 95.06 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.24 & \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.13 & \cellcolor[HTML]{005321} \color[HTML]{f1f1f1} 97.97 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 53.12 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.37 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.42 & \cellcolor[HTML]{dcf2d7} \color[HTML]{000000} 66.44 & \cellcolor[HTML]{e9f7e5} \color[HTML]{000000} 63.90 \\
% GIN+EdgeUpdates & 
% \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.30 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.74 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.70 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.13 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 32.58 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 55.91 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 54.65 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 47.62 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 49.68 & \cellcolor[HTML]{d0edca} \color[HTML]{000000} 68.54 & \cellcolor[HTML]{e7f6e2} \color[HTML]{000000} 64.64 \\
GIN+Ports \citep{sato2019approximation_port_numbers} & 
\cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.47 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 45.00 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.59 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 41.51 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 27.79 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 56.11 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 42.68 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 41.11 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 44.99 & \cellcolor[HTML]{d3eecd} \color[HTML]{000000} 67.99 & \cellcolor[HTML]{e1f3dc} \color[HTML]{000000} 65.76 \\
\midrule
GIN+ReverseMP \citep{jaume2019edgnnbidirecibmmaria} & 
\cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.87 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.08 & \cellcolor[HTML]{006d2c} \color[HTML]{f1f1f1} 94.99 & \cellcolor[HTML]{006b2b} \color[HTML]{f1f1f1} 95.25 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 35.96 & \cellcolor[HTML]{e9f7e5} \color[HTML]{000000} 63.85 & \cellcolor[HTML]{ccebc6} \color[HTML]{000000} 69.09 & \cellcolor[HTML]{d7efd1} \color[HTML]{000000} 67.44 & \cellcolor[HTML]{bee5b8} \color[HTML]{000000} 71.23 & \cellcolor[HTML]{e0f3db} \color[HTML]{000000} 65.83 & \cellcolor[HTML]{def2d9} \color[HTML]{000000} 66.18 \\
{\ +Ports} & 
\cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.41 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.35 & \cellcolor[HTML]{005020} \color[HTML]{f1f1f1} 98.51 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.16 & \cellcolor[HTML]{f7fcf5} \color[HTML]{000000} 39.15 & \cellcolor[HTML]{ebf7e7} \color[HTML]{000000} 63.58 & \cellcolor[HTML]{cdecc7} \color[HTML]{000000} 69.00 & \cellcolor[HTML]{c4e8bd} \color[HTML]{000000} 70.35 & \cellcolor[HTML]{a0d99b} \color[HTML]{000000} 75.04 & \cellcolor[HTML]{d4eece} \color[HTML]{000000} 67.84 & \cellcolor[HTML]{e1f3dc} \color[HTML]{000000} 65.78 \\
{\ +EgoIDs (Multi-GIN)} & 
\cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.48 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.09 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.62 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.32 & \cellcolor[HTML]{004c1e} \color[HTML]{f1f1f1} 98.97 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.46 & \cellcolor[HTML]{17813d} \color[HTML]{f1f1f1} 91.60 & \cellcolor[HTML]{48ae60} \color[HTML]{f1f1f1} 84.23 & \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.42 & \cellcolor[HTML]{05712f} \color[HTML]{f1f1f1} 94.33 \\
% +EdgeUpdates & 
% \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.55 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.76 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.37 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.73 & \cellcolor[HTML]{2d954d} \color[HTML]{f1f1f1} 88.38 & \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.81 & \cellcolor[HTML]{005522} \color[HTML]{f1f1f1} 97.82 \\
\midrule
% GAT+Adaptations & 
% \cellcolor[HTML]{005020} \color[HTML]{f1f1f1} 98.44 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.66 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.18 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.11 & \cellcolor[HTML]{005221} \color[HTML]{f1f1f1} 98.28 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.42 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.35 & \cellcolor[HTML]{026f2e} \color[HTML]{f1f1f1} 94.55 & \cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} 91.75 & \cellcolor[HTML]{218944} \color[HTML]{f1f1f1} 90.21 & \cellcolor[HTML]{79c67a} \color[HTML]{000000} 79.52 \\
Multi-GAT & 
\cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.68 & \cellcolor[HTML]{005120} \color[HTML]{f1f1f1} 98.36 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.28 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.33 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.61 & \cellcolor[HTML]{004c1e} \color[HTML]{f1f1f1} 98.93 & \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.90 & \cellcolor[HTML]{006529} \color[HTML]{f1f1f1} 95.82 & \cellcolor[HTML]{16803c} \color[HTML]{f1f1f1} 91.81 & \cellcolor[HTML]{005f26} \color[HTML]{f1f1f1} 96.66 & \cellcolor[HTML]{359e53} \color[HTML]{f1f1f1} 86.92 \\
Multi-PNA & 
\cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.64 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.25 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.41 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.54 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.49 & \cellcolor[HTML]{005924} \color[HTML]{f1f1f1} 97.46 & \cellcolor[HTML]{2a924a} \color[HTML]{f1f1f1} 88.75 & \cellcolor[HTML]{004a1e} \color[HTML]{f1f1f1} 99.07 & \cellcolor[HTML]{005e26} \color[HTML]{f1f1f1} 96.77 \\
Multi-GIN+EU & 
\cellcolor[HTML]{00471c} \color[HTML]{f1f1f1} 99.55 & \cellcolor[HTML]{00481d} \color[HTML]{f1f1f1} 99.53 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.76 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.77 & \cellcolor[HTML]{00491d} \color[HTML]{f1f1f1} 99.37 & \cellcolor[HTML]{00451c} \color[HTML]{f1f1f1} 99.71 & \cellcolor[HTML]{004e1f} \color[HTML]{f1f1f1} 98.73 & \cellcolor[HTML]{006729} \color[HTML]{f1f1f1} 95.73 & \cellcolor[HTML]{2d954d} \color[HTML]{f1f1f1} 88.38 & \cellcolor[HTML]{004d1f} \color[HTML]{f1f1f1} 98.81 & \cellcolor[HTML]{005522} \color[HTML]{f1f1f1} 97.82 \\
\bottomrule
\end{tabular}
}
\endgroup

